TD-Regularized Actor-Critic Methods

Actor-critic methods can achieve incredible performance on difficult reinforcement learning problems, but they are also prone to instability. This is partly due to the interaction between the actor and critic during learning, e.g., an inaccurate step taken by one of them might adversely affect the other and destabilize the learning. To avoid such issues, we propose to regularize the learning objective of the actor by penalizing the temporal difference (TD) error of the critic. This improves stability by avoiding large steps in the actor update whenever the critic is highly inaccurate. The resulting method, which we call the TD-regularized actor-critic method, is a simple plug-and-play approach to improve stability and overall performance of the actor-critic methods. Evaluations on standard benchmarks confirm this.

==> bibliography_abbrv <==
@Article	- journal paper
@InProceedings	- conference paper and workshops
@Book		- book
@InCollection	- book chapter
@Other		- online and arXiv

If a name has dashes or is composed by two names, put it into curly brackets (e.g., {John-Doe} or {Soncini Sessa}).
The same if a word needs to be upper case (e.g., {PCA}).

To avoid pag, publisher, organizer, etc... you need to redefine bibliography style.
Use \bibliographystyle{myIEEEtran.bst} that already removes some of them (the useless and ugly ones).





  Booktitle                = {Proceedings of the Joint Conference on Machine Learning and Knowledge Discovery in Databases ({ECML/PKDD})},
  Booktitle                = {Proceedings of the International Conference on Autonomous Agents and Multi-Agent Systems (AAMAS)},
  Booktitle                = {Proceedings of the International Conference on Robotics and Automation (ICRA)},
  Booktitle                = {Proceedings of the International Conference on Intelligent Robots and Systems (IROS)},
  Booktitle                = {Proceedings of Robotics: Science and Systems (R:SS)},
  Booktitle                = {Proceedings of the American Control Conference (ACC)},
  Booktitle                = {Advances in Neural Information Processing Systems (NIPS)},
  Booktitle                = {Proceedings of the International Conference on Machine Learning (ICML)},
  Booktitle                = {Proceedings of International Conference on Machine Learning and Applications (ICMLA)},
  Booktitle                = {Proceedings of the International Symposium on Artificial Intelligence and Mathematics (ISAIM)},
  Booktitle                = {Proceedings of the Conference on Artificial Intelligence (AAAI)},
  Booktitle                = {Proceedings of the International Joint Conference on Neural Networks (IJCNN)},
  Booktitle                = {Proceedings of the European Conference on Machine Learning (ECML)},
  Booktitle                = {Proceedings of International Symposium on Approximate Dynamic Programming and Reinforcement Learning (ADPRL)},
  Booktitle                = {Proceedings of the International Conference on Humanoid Robots (HUMANOIDS)},
  Booktitle                = {Proceedings of the International Conference on Artificial Neural Networks (ICANN)},
  Booktitle                = {Proceedings of the Genetic and Evolutionary Computation Conference (GECCO)},
  Booktitle                = {Proceedings of the Australasian Conference on Artificial Intelligence (AI)},
  Booktitle                = {Proceedings of the European Conference on Artificial Intelligence (ECAI)},
  Booktitle                = {Proceedings of the International Conference on Acoustics, Speech, and Signal Processing (ICASSP)},
  Booktitle                = {Proceedings of the International Joint Conference on Artifical Intelligence (IJCAI)},
  Booktitle                = {Proceedings of the Conference on Decision and Control (CDC)},
  Booktitle                = {Proceedings of the International Conference on Networking, Sensing and Control (ICNSC)},
  Booktitle                = {Proceedings of the Annual Symposium on Theoretical Aspects of Computer Science (STACS)},
  Booktitle                = {Proceedings of the International Conference on Artificial Intelligence and Statistics (AISTATS)},
  Booktitle                = {Proceedings of the Conference on Uncertainty in Artificial Intelligence (UAI)},
  Booktitle                = {Proceedings of the Conference on Learning Theory (COLT)},
  Booktitle                = {Proceedings of the International Conference on Intelligent Autonomous Systems (IAS)},
  Booktitle                = {Proceedings of the International Conference on Fuzzy Systems},
  Booktitle                = {Proceedings of the International Conference on Agents and Artificial Intelligence (ICAART)},
  Booktitle                = {Proceedings of the AIAA/ISSMO Multidisciplinary Analysis Optimization Conference},
  Booktitle                = {Advances in Artificial Intelligence},
  Booktitle                = {Proceedings of the Symposium Series on Computational Intelligence (SSCI)},
  Booktitle                = {Congress on Evolutionary Computation},
  Booktitle                = {Proceedings of the International Conference on Learning Representations (ICLR)},

  Booktitle                = {Recent Advances in Reinforcement Learning},
  Booktitle                = {Proceedings of the AAAI Workshop on Intelligent Robotic Systems},
  Booktitle                = {Proceedings of the International Conference on Simulation of Adaptive Behavior (SAB)},

  Journal                  = {K{\"u}nstliche Intelligenz (KI)},
  Journal                  = {Control Systems},
  Journal                  = {Journal of Machine Learning Research (JMLR)},
  Journal                  = {Foundations and Trends in Robotics},
  Journal                  = {Transactions on Autonomous Mental Development},
  Journal                  = {Autonomous Robots},
  Journal                  = {Robotics},
  Journal                  = {Robotics and Autonomous Systems},
  Journal                  = {The International Journal of Robotics Research (IJRR)},
  Journal                  = {Adaptive Behavior Journal},
  Journal                  = {Annals of Operations Research},
  Journal                  = {Neural Networks},
  Journal                  = {Neurocomputing},
  Journal                  = {Neural Computation},
  Journal                  = {Engineering Optimization},
  Journal                  = {Theoretical Computer Science},
  Journal                  = {Discrete Event Dynamic Systems},
  Journal                  = {Journal of Artificial Intelligence Research (JAIR)},
  Journal                  = {Journal of Control Theory and Applications},
  Journal                  = {International Journal of Computers, Systems and Signals},
  Journal                  = {Water Resources Research},
  Journal                  = {Machine Learning},
  Journal                  = {Studia Scientiarium Mathematicarum Hungarica},
  Journal                  = {Mathematical Methods of Operations Research},
  Journal                  = {International Journal for Numerical Methods in Engineering},
  Journal                  = {Information Theory},
  Journal                  = {Structural and Multidisciplinary Optimization},

